Boosting Online 3D Multi-Object Tracking through Camera-Radar Cross Check

In the domain of autonomous driving, the integration of multi-modal perception techniques based on data from diverse sensors has demonstrated substantial progress. Effectively surpassing the capabilities of state-of-the-art single-modality detectors through sensor fusion remains an active challenge. This work leverages the respective advantages of cameras in perspective view and radars in Bird's Eye View (BEV) to greatly enhance overall detection and tracking performance. Our approach, Camera-Radar Associated Fusion Tracking Booster (CRAFTBooster), represents a pioneering effort to enhance radar-camera fusion in the tracking stage, contributing to improved 3D MOT accuracy. The superior experimental results on the K-Radaar dataset, which exhibit 5-6% on IDF1 tracking performance gain, validate the potential of effective sensor fusion in advancing autonomous driving.

==> tex/4_exp.tex <==
\section{Experiments} \label{section_exp}

\paragraph{Datasets and Evaluation Metrics.}

We evaluate our method on the K-Radar~\cite{paek2023kradar} and CRUW3D~\cite{cruw3d} datasets as they uniquely provide radar tensors and camera video frames with 3D object bounding box and tracking annotations in diverse driving scenarios. 
We do not use other databases solely containing radar point clouds, such as nuScenes\cite{nuscenes}, TJ4DRadSet\cite{Zheng_2022} and RadarScenes\cite{schumann2021radarscenes}. 
As indicated by the results on these datasets, the performance of 3D perception using radar point clouds is not comparable with that of using the camera unless high-end radar equipment like RADIATE\cite{sheeny2021radiate} is employed. 
K-Radar encompasses scenarios, characterized by varying illumination, weather conditions, and road structures. 
It offers synchronized data, including LiDAR point clouds, 4D radar tensors, and camera images. 
It is divided into approximately 17.5k training and 17.5k testing frames from its raw continuous sequences.
CRUW3D comprises 66K synchronized camera frames, 3D radar tensors, and LiDAR point clouds in different lighting conditions. 
In CRUW3D, we select ten scenarios which contain 18K frames in total, and divide half of the frames for training and the other half for testing.
Table~\ref{tab:trackerPerformance} shows that there is a marginal difference in camera's performance between the two datasets. 
We attribute this observation to the different characteristics of the two datasets. 
Compared to K-Radar, CRUW3D's driving scenes are in good weather, which favors camera-based perception methods.
We adopt MOTA and IDF1 in evaluation to measure 3D object tracking performance.

\paragraph{Detectors.}
 Following the paradigm of tracking by detection, 
 we implement advanced monocular and radar-based 3D object detectors to lay a firm foundation for the subsequent tracking stage. 
 We choose DD3D~\cite{park2021pseudolidar} as our camera's baseline detector, as it is renowned for its superiority in monocular 3D object detection owing to its strong depth-inferring ability. 
 DD3D provides two backbones pre-trained on large-scale depth images~\cite{packnet}.
 We use the DLA-34~\cite{8578353} pre-trained backbone and fine-tune the detector on the K-Radar and CRUW3D datasets. 
 Since DD3D does not infer re-ID embedding features, we apply the publicly available YOLOX\cite{ge2021yolox} detector to extract re-ID features from cropped image regions projected by DD3D's detected 3D bounding boxes. 
 We pick CenterRadarNet~\cite{cheng2023centerradarnet} as our radar's baseline 3D object detector. 
 CenterRadarNet is a joint architecture for 3D object detection and tracking. 
 It learns discriminative representation from 4D radar tensors and favors object localization and re-identification (re-ID) tasks. 
 We employ the same detectors across all experiments. 
%Andy so strong 

\paragraph{Results.} Table~\ref{tab:trackerPerformance} presents the performance of methods on K-Radar and CRUW3D. We use several MOT algorithms for comparison. In CRAFTBooster, we employ ByteTrack and BOTSORT as online trackers within the \textbf{Inner-modality Matching Module}. 
The results demonstrate that our model enhances the performance of the camera's and radar's baseline models. 
It is worth mentioning that the K-Radar encompasses numerous adverse weather conditions, where vehicle objects are entirely obscured in the images. 
Thus, the performance of the camera's perception model, especially compared with the result from the radar's perception model, is significantly lower. 
In our experiments, CRAFTBooster performs best when utilizing BOTSORT as the online tracker in \textbf{Inner-modality Matching Module}. 
Note that our approach surpasses the better modality's performance by 3.6\% to 4.8\% in IDF1. 


\begin{table}[]
    \centering
    % \setlength\tabcolsep{3pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{cc cc|cc}
        \toprule
        \multirowcell{2}{Tracking\\Method}&\multirowcell{2}{Modality}&\multicolumn{2}{c}{K-Radar}&\multicolumn{2}{c}{CRUW3D}\\
        & & IDF1$\uparrow$ & MOTA$\uparrow$ & IDF1$\uparrow$ & MOTA$\uparrow$ \\
        \midrule

        \multirow{2}{*}{OC-SORT\cite{cao2023observationcentric}}& Camera & 39.0 & 8.4 & 70.6 & 69.2 \\
        &Radar & 56.0 & 36.0 & 51.8 & 41.3 \\
        \midrule
        
        \multirow{2}{*}{StrongSORT*\cite{du2023strongsort}}& Camera & 40.3 & 18.2 & 69.8 & 69.2 \\
        &Radar & 51.5 & 38.1 & 51.9& 41.6 \\
        \midrule
        
        \multirow{2}{*}{ByteTrack\cite{zhang2022bytetrack}}& Camera & 41.4 & 19.1 & 71.3 & 69.7  \\
        &Radar & 52.5 & 42.5 & 53.5 & 41.8 \\
        \rowcolor[gray]{0.9}
        CRAFTBooster & Radar+Camera & 58.3 &44.7& 72.0 & 69.8 \\
        \midrule
        
        \multirow{2}{*}{BOTSORT\cite{aharon2022botsort}}&Camera & 45.3& 20.0 & 71.1 & 69.4 \\
        & Radar & 55.3 & 41.1 & 50.6 & 39.6 \\
        \rowcolor[gray]{0.9}
        \textbf{CRAFTBooster}& Radar+Camera & \textbf{59.5}& \textbf{44.9} & 74.2 & 69.4 \\

        \bottomrule
    \end{tabular}}
    \caption{Overall Performance on K-Radar and CRUW3D Dataset. We implement our method on both ByteTrack and BOTSORT. StrongSORT*: We implement StrongSORT with some modifications, such as removing AFLink, ECC and also BoT( We replace it with our own detector).}
    \label{tab:trackerPerformance}
\end{table}

% \begin{table}[!h]
%     \centering
%     % \setlength\tabcolsep{3pt}
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{cc cc|cc}
%         \toprule
%         \multirowcell{2}{Tracking\\Method}&\multirowcell{2}{Modality}&\multicolumn{2}{c}{K-Radar}&\multicolumn{2}{c}{CRUW3D}\\
%         & & IDF1$\uparrow$ & MOTA$\uparrow$ & IDF1$\uparrow$ & MOTA$\uparrow$ \\
%         \midrule

%         \multirow{2}{*}{OC-SORT\cite{cao2023observationcentric}}& Camera & 39.0 & 8.4 & 70.6 & 69.2 \\
%         &Radar & 56.0 & 36.0 & 51.8 & 41.3 \\
%         \midrule
        
%         \multirow{2}{*}{StrongSORT*\cite{du2023strongsort}}& Camera & 40.3 & 18.2 & 69.8 & 69.2 \\
%         &Radar & 51.5 & 38.1 & 51.9& 41.6 \\
%         \midrule
        
%         \multirow{2}{*}{ByteTrack\cite{zhang2022bytetrack}}& Camera & 41.4 & 19.1 & 71.3 & 69.7  \\
%         &Radar & 52.5 & 42.5 & 53.5 & 41.8 \\
%         \midrule
        
%         \multirow{2}{*}{BOTSORT\cite{aharon2022botsort}}&Camera & 45.3& 20.0 & 71.1 & 69.4 \\
%         & Radar & 55.3 & 41.1 & 50.6 & 39.6 \\
%         \midrule
        
%         \textbf{Ours w/ ByteTrack}& Radar+Camera & \textbf{58.3} & \textbf{44.7} & 72.0 & 69.8 \\
%         \textbf{Ours w/ BOTSORT}& Radar+Camera & \textbf{59.5}& \textbf{44.9} & 74.2 & 69.4 \\

%         \bottomrule
%     \end{tabular}}
%     \caption{Overall Performance on K-Radar and CRUW Dataset. We implement our method on ByteTrack and BOTSORT, which are denoted as Ours-ByteTrack and Ours-BOTSORT. StrongSORT*: We implement StrongSORT with some modifications, such as removing AFLink, ECC and also BoT( We replace it with our own detector), which may cause unfairness.}
%     \label{tab:trackerPerformance}
% \end{table}

Our method enables each modality to obtain a refined tracklet set after \textbf{Cross-modality Check Module}. 
This tracklet set can be viewed as the outcome of enhanced performance complemented by the other modality. 
In Table~\ref{tab:CR_Refined}, we discuss the results of camera and radar separately. 
In both the radar and camera refined tracklets, we observe an increase of 3-8\% in IDF1 compared to performance of the original tracker. From the number of false negatives (FNs), it is evident that our module effectively recovers the missing data, although it may inveitably introduce some invalid data in false positives (FPs). It is also worth mentioning that the performance of the refined tracklet set can even surpass the final results of CRAFTBooster. The primary goal of the \textbf{Multi-modality Fusion Module} is to identify a comparable modality that aligns closely with the better-performing sensor modality in scenarios where additional information about sensor conditions is lacking. 

\begin{table}[!h]
    \centering
    % \setlength\tabcolsep{3pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
         \makecell[c]{Modality}&\makecell[c]{Tracking\\Method}& \makecell[c]{IDF1$\uparrow$} & \makecell[c]{MOTA$\uparrow$\\ }&FP$\downarrow$&FN$\downarrow$&IDs$\downarrow$\\
        \midrule
        \multirowcell{6}{Radar}&OC-SORT\cite{cao2023observationcentric}& 56.0 & 36.0 & 4,554 & 14,327 &640\\ 
        &StrongSORT*\cite{du2023strongsort} & 51.5& 38.1 & 3,675 & 15,054 &422\\ 
        &ByteTrack\cite{zhang2022bytetrack} & 52.5 & 42.5 & 2,557 & 14,824 & 415 \\
        &BOTSORT\cite{aharon2022botsort}& 55.3 & 41.1 & 2,180 & 15,640 & 423 \\
        \rowcolor[gray]{0.9}
        &\textbf{Ours w/ ByteTrack}& 61.1 & 46.9 & 3,212 & 12,941 & 305 \\
        \rowcolor[gray]{0.9}
        &\textbf{Ours w/ BOTSORT}& \textbf{63.4} & \textbf{47.2} & 3,316 & 12,775 & 266 \\
        \midrule
        \multirowcell{6}{Camera}&OC-SORT\cite{cao2023observationcentric}& 39.1 & 8.4 & 8,725 & 18,332 & 1,332\\ 
        &StrongSORT*\cite{du2023strongsort} & 40.3 & 18.2& 3,541 & 21,341 &425\\ 
        &ByteTrack\cite{zhang2022bytetrack} & 41.4 & 19.1 & 6,335 & 18,338 & 389 \\ 
        &BOTSORT\cite{aharon2022botsort}& 45.3 & 20.0 & 5,824 & 18,648 & 306 \\
        \rowcolor[gray]{0.9}
        &\textbf{Ours w/ ByteTrack}& 46.9 & 21.2 & 6502 & 17,579 & 315 \\
        \rowcolor[gray]{0.9}
        &\textbf{Ours w/ BOTSORT}& \textbf{48.0} & \textbf{21.9} & 6,332 & 17,525 & 326 \\
        
        
        \bottomrule
    \end{tabular}}
    \caption{Performance Comparison of Radar and Camera Refined Tracklet Set with Baselines. We incorporate ByteTrack and BOTSORT in our CRAFTBooster), denoted as Ours w/ByteTrack and Ours w/BOTSORT. StrongSORT*: We implement StrongSORT with some modifications: removing AFLink, ECC, and BoT( We replace it with our own detector).}
    \label{tab:CR_Refined}
\end{table}

In various weather conditions, each sensor modality is affected by lighting and environmental factors, resulting in degradation in performance, as shown in Fig~\ref{fig:Weather_IDF1}. In favorable weather conditions with normal lighting, the camera exhibits superior performance. Conversely, in other adverse environments, radar outperforms the camera. During rain/sleet, the camera often struggles due to blurred images, resulting in the poorest performance. As the result, it is evident that our method enhances performance across various weather conditions, surpassing the best-performing modality in the given environment.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/Weather_IDF1.pdf}
    % \includegraphics[width=0.9\linewidth]{fig/weather.pdf} % wenhao
    \caption{Comparison of IDF1\% under various weather conditions on K-Radar dataset. BOTSORT-Camera and BOTSORT-Radar mean that the tracking result is from BOTSORT with different kind of senso. The online trackers in CRAFTBooster are based on BOTSORT in two modalities.}
    \label{fig:Weather_IDF1}
\end{figure}

Furthermore, we aim to understand how much each modality could be reinforced by the other modality using our method across various weather conditions. Therefore, we calculate the difference in values using the \textbf{Recall} metric, as illustrated in Fig~\ref{fig:Recall_Weather_1}. The results reveal that under normal weather conditions, radar can be enhanced by 9-13\% in Recall through the camera modality. The significant changes in true positives (TPs) clearly indicate the strength of improvement. In adverse weather conditions, such as Rain/Sleet or Fog/Snow, camera can also be enhanced by approximately 6\% through radar. As previously mentioned, the fusion results align closely with the outcomes of the better-performing modality.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/Recall_Weather_1.pdf}
    % \includegraphics[width=0.9\linewidth]{fig/recall.pdf} % wenhao
    \caption{\textbf{Recall} Metric under various weather conditions. Radar Refined and Camera Refined denote the output after \textbf{the Cross-modality Check Module.}}
    \label{fig:Recall_Weather_1}
\end{figure}

Camera detection remains stable under normal conditions in Fig~\ref{fig:vis_exp}, but exhibits issues with miss-detection in inclement weather, confirming in Fig~\ref{fig:Recall_Weather_1}. It's worth noting that we found that the primary factors influencing radar results are the density of vehicles or the abundance of surrounding objects, possibly tied to equipment resolution. 

 % We believe that the concept presented in this article holds the potential for a long-term research vision. The current method still possess certain limitations and possibilities for further development. The primary challenge confronted by our method is that the fusion result cannot surpass all the refined tracklet set after Cross-modality Check Module, as evidenced by the comparison of results in Table \ref{tab:trackerPerformance} and Table \ref{tab:CR_Refined}.  Through the visualization of results, we find that the main issue lies in the quantity of false positives (FPs), which can also be observed in Table \ref{tab:CR_Refined}. The FPs of refined tracklets on each modality are more than the the origional tracker. It remains difficult to determine whether these instances truly exist  based on limited information from the other modality. We expect that this issue can be overcome by extracting additional information from the raw data of each modality in the future.

\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{fig/vis_exp.pdf}
    % \includegraphics[width=1\linewidth]{fig/vis_exp_v2.pdf}

    \caption{Samples from the result under various weather conditions on K-Radar dataset. We visualize the fusion tracking result(b), comparing with BOTSORT's result on camera(a) and radar(c). }
    \label{fig:vis_exp}
\end{figure*}


